Sublinear Time Approximation of Text Similarity Matrices

We study algorithms for approximating pairwise similarity matrices that arise in natural language processing. Generally, computing a similarity matrix for $n$ data points requires $\Omega(n^2)$ similarity computations. This quadratic scaling is a significant bottleneck, especially when similarities are computed via expensive functions, e.g., via transformer models. Approximation methods reduce this quadratic complexity, often by using a small subset of exactly computed similarities to approximate the remainder of the complete pairwise similarity matrix. Significant work focuses on the efficient approximation of positive semidefinite (PSD) similarity matrices, which arise e.g., in kernel methods. However, much less is understood about indefinite (non-PSD) similarity matrices, which often arise in NLP. Motivated by the observation that many of these matrices are still somewhat close to PSD, we introduce a generalization of the popular Nystr\"{o}m method to the indefinite setting. Our algorithm can be applied to any similarity matrix and runs in sublinear time in the size of the matrix, producing a rank-$s$ approximation with just $O(ns)$ similarity computations. We show that our method, along with a simple variant of CUR decomposition, performs very well in approximating a variety of similarity matrices arising in NLP tasks. We demonstrate high accuracy of the approximated similarity matrices in the downstream tasks of document classification, sentence similarity, and cross-document coreference.

==> 005application_details.tex <==
\section{Application details}\label{sec: application details}

In this section, we describe how our generalized \nystrom algorithm can be used in two applications of document and sentence similarity. The first application is document similarity using word movers distance \cite{kusner2015word}. We demonstrate the our proposed \nystrom method can accurately approximate the pairwise similarity matrix. We further show that \nystrom provides embedded representations of the documents which respect the pairwise similarities given by word movers distances. We show that these can be used as features to train a supervised classifier. The second application
is modeling sentence similarity with cross encoder
BERT models \cite{devlin2018bert}. Both applications are selected because the respective similarity functions lead to matrices which are not necessarily PSD and the similarity functions are expensive to compute.

\subsection{Document similarity \& classification with word movers distance}\label{sec: approximate wmd}

Word mover's distance (WMD) \cite{kusner2015word} is a similarity between documents which measures how well words in one document aligns (i.e., matches) with the words in another document. The words of the documents are typically represented by vectors and the cost of alignment is based on the distances between matched words.

In this application, our dataset $\mathcal{X}$, consists of documents $x \in \mathcal{X}$ with $|x|$ words each.
 Using a normalized bag of words representation, each document is represented as a vector in $\mathbb{R}^m$, where $m$ is the size of the dictionary. Let word $i$ in the dictionary appear $q_i$ times in the document $x$ then $d^x_i = \frac{q_i}{\sum_{k=1}^n q_k}$. For each of these words, we assume that we have  representations in the form of vectors (like \emph{word2vec} \cite{mikolov2013efficient}). Let matrix $C$ be defined such that $C_{ij} = \|x_i-x_j\|_2$, where $x_i, x_j$ are $i^{th}$ and $j^{th}$ words of dictionary. Thus each entry in $C_{ij}$ consists of the Euclidean distance between two words $x_i, x_j$ in their embedding space. To compute the cost of aligning the two documents $x, y$, we allow each word in $x$ to be transformed in whole or part to any word $y$. Define $F \in \mathbb{R}^{|x|\times |y|}$ as a matrix such that $F_{ij} \in [0,1]$ indicates what fraction of the $i^{th}$ word in $x$ transforms into (or aligns with) the $j^{th}$ word $y$. To ensure the whole document $x$ is transformed into $y$ and vice versa we require that $\sum_j F_{ij} = d^x_i$ and also $\sum_i F_{ij} = d^x_j$. Define $\mathcal{F}$ be the set of all such matrices $F$. The WMD between $x, y$ is defined as

Observe that the computational complexity of WMD to compare two documents of maximum length $L$ is $\mathcal{O}(L^3 \log(L))$ \cite{kusner2015word}. Thus it is expensive to compute for each pair of documents, motivating approximate methods to compute the pairwise similarity matrix. Additionally we empirically observe that this measure does not necessarily lead to a PSD matrix. While we don't have a analytical proof for this, we observe that the related Wasserstein metric leads to non PSD matrices \cite{courty2017learning}.


\textbf{Baseline - Monte Carlo approximations}. In \cite{wu2018word}, a Monte Carlo approximation to a \emph{kernelized} WMD is achieved which has a run-time of $\mathcal{O}(nRL\log(L))$ computations, where $R$ is the number of trials in Monte Carlo approximation required to arrive at \emph{good} random features. In \cite{wu2018word}, the authors construct a PSD matrix using the WMD via a infinite dimensional feature map constructed using WMD of all documents to randomly generated features. We refer to this matrix as kernelized WMD. The approximation is then used to compute document embedding using Random Features approximation to the PSD. This is called Word Mover's Embedding (WME). Experiments show that apart from being much faster from generating features, WME outperforms true WMD's linear SVM performance considering large rank is used for approximation of the WMD kernel. For small rank approximation WME achieves comparable results to classifiers generated using KNN and WMD.

\textbf{Proposed approach - \nystrom method}. WME's random features are drawn uniformly at random from $\mathbb{R}^{D_{\max}}$ where $D_{\max}$ is the maximum size of any document in the dataset.
Instead we decided to try generalized \nystrom on the problem of approximating a similarity metric derived from WMD. The idea being: since \nystrom is data driven, the approximation will only depend on how the data is distributed and which samples are chosen to represent the whole dataset. 
We define the similarity function $\Delta: \mathcal{X}\times\mathcal{X}\to\mathbb{R}$ which uses WMD to compute distances, as follows: 
% \vspace{-0.25cm}
\begin{align}\label{eq: WMD kernel}
    \Delta(x, \omega) = \exp(-\gamma \text{WMD}(x, \omega))~\forall~x,\omega\in\mathcal{X},
\end{align}
where WMD is calculated using \ref{eq: WMD distance}. Thus if we input set of datapoints in $x$ and landmark points in $\omega$, then $\Delta$ should yield an exponentiated $-\gamma$ times the WMD distance matrix among the points $x$ and $\omega$. The resulting algorithm to extract WME features using \nystrom approximation is detailed in Algorithm \ref{alg:nwme}.

\input{NWME}

\Cam{Generally, significantly shorten description of the setup, and also remove pseudocode. Just describe in words what the similarity function is and how you then apply Algorithm \ref{alg:generalized_nystrom}. Same with the second on BERT.}

Algorithm \ref{alg:nwme} instantiates the WMD kernel function, which is the distance function used in Algorithm \ref{alg:generalized_nystrom}. We use Algorithm \ref{alg:nwme} to compute the feature vectors $\bv{Z}$. These vectors are then used to train a SVM based linear classifier. The sample indices $S_s$ is used as landmark points for generating the \nystrom WME features for validation and test data points.  
 
\subsection{Cross-encoder sentence similarity}\label{sec: approximate bert}

The second set of problems we are interested in is simplifying computation for models like cross-encoder BERT \cite{devlin2018bert}. A cross-encoder model is a neural network that takes in two sentences/documents and computes a similarity score. The score so computed is not necessarily a metric since it may or may not follow transitive and reflexive properties. Thus cross-encoder models are generally black box simulation giving us no intuition on the how the similarity scores are computed. Moreover the number of such computations to evaluate the similarity scores is large. Since \nystrom based approximation can approximate matrices without having to access all entries of the matrix, the required number of computation can be drastically reduced. 

We consider three sentence similarity tasks part of the GLUE (citation) benchmark: sentence matching (STS-B) \cite{stsb}, semantic equivalence (MRPC) \cite{mrpc} and entailment (RTE) \cite{rte}. Observe that computing a single element of the pairwise matrix requires running the cross-encoder model on the pair of inputs. The running time for this is around 0.004 seconds on a RTX 3090 GPU and takes about 10 hours for datasets of size around 900000 samples, which is prohibitively expensive.

The similarities computed using the neural networks are generally conditional and non-symmetric. The set of problems we consider are reflexive in nature\footnote{If matrix $\bv K$ are not symmetric we can always symmetrize by $(\bv K + \bv K^T)/2$}. As such to account for noise in data we can consider computing a symmetrized similarity matrix. Thus the similarity function in this case is:
\begin{align}
    \Delta(x, \omega) = \textsf{CE\_BERT}(x, \omega)~\forall~x,\omega\in\mathcal{X},
\end{align}
where $\textsc{CE\_BERT}$ computes cross-encoder  similarity between sentence pairs $x, \omega$.
The resulting algorithm is thus: 

\input{NWME_BERT}

In test time we thus only need to compute $\mathcal{O}(s)$ similarities to the landmark points which saves us the computation time of running the cross-encoder BERT for $\mathcal{O}({n^2})$ times. 


==> zoomed_plots.tex <==
\begin{figure*}[ht]
\vspace{-10cm}
% \centering
    % \begin{subfigure}
    \centering%
    \includegraphics[width=0.48\textwidth]{figures/zoomed_plots/PSD.pdf}
    \vspace{-.1cm}
    \includegraphics[width=0.48\textwidth]{figures/zoomed_plots/twitter.pdf}
    \vspace{-.1cm}
    \includegraphics[width=0.48\textwidth]{figures/zoomed_plots/stsb.pdf}
    \vspace{-.1cm}
    \includegraphics[width=0.48\textwidth]{figures/zoomed_plots/mrpc.pdf}
    \caption{\textbf{Zoomed in approximation error plots.} For better visualization of Figure \ref{fig: naive nystrom vs CUR variants}, here we present the zoomed in version of the plots. As stated earlier, if a method does not appear, it may be that it had large error which is out of range of the y-axis. In case of the PSD matrix and similarity matrix of Twitter, several methods overlap and hence and not distinctly visible.}
    \label{fig: zoomed plots}
\end{figure*}
